MOST-Net: A Memory Oriented Style Transfer Network for Face Sketch Synthesis

Face sketch synthesis has been widely used in multi-media entertainment and law enforcement. Despite the recent developments in deep neural networks, accurate and realistic face sketch synthesis is still a challenging task due to the diversity and complexity of human faces. Current image-to-image translation-based face sketch synthesis frequently encounters over-fitting problems when it comes to small-scale datasets. To tackle this problem, we present an end-to-end Memory Oriented Style Transfer Network (MOST-Net) for face sketch synthesis which can produce high-fidelity sketches with limited data. Specifically, an external self-supervised dynamic memory module is introduced to capture the domain alignment knowledge in the long term. In this way, our proposed model could obtain the domain-transfer ability by establishing the durable relationship between faces and corresponding sketches on the feature level. Furthermore, we design a novel Memory Refinement Loss (MR Loss) for feature alignment in the memory module, which enhances the accuracy of memory slots in an unsupervised manner. Extensive experiments on the CUFS and the CUFSF datasets show that our MOST-Net achieves state-of-the-art performance, especially in terms of the Structural Similarity Index(SSIM).

==> MOST-NET ICPR2022/MemoryDictionary.tex <==
\subsection{Memory Dictionary}
%照应一下A中的命名呗,尽量小模块不用networks，和大的网络冲突
\label{memory}
\subsubsection{Memory Mechanism}
We define the memory mechanism as a dictionary $M$ holding pairs of the key $k_{i}\in \mathbb{R}^{c}$ and value  $v_{i}\in \mathbb{R}^{c}$, which represents the photo feature slots and its corresponding sketch feature slots.
%学术论文最好不用动名词doing开头的句子，主谓宾， 谁干了什么，这种最好
Each entry $(k_{i},v_{i})$ of $M$ represents a feature mapping from photo domain to sketch domain. 
Therefore, a dictionary $M$ containing K items can be described in the following:
\begin{equation}\label{1}
M = \left \{ (k_{i},v_{i})\mid k_{i},v_{i}\in\mathbb{R}^{c},i=1,2,3\cdots ,K \right \}
\end{equation}

Given input photo features $F_{p}$ and sketch features $F_{s}$, we divide them into a number of slots:
\begin{equation}\label{2}
F_{p}= \left \{ f_{1}, f_{2},f_{3},\cdots f_{N}\right \},f_{i}\in \mathbb{R}^{c} 
\end{equation}
\begin{equation}\label{3}
F_{s}= \left \{ s_{1}, s_{2},s_{3},\cdots s_{N}\right \},s_{i}\in \mathbb{R}^{c}
\end{equation}
where $N$ is the number of slots (feature map size), $c$ denotes the dimension of the each slot. Since these slots are intended to interact with Memory Dictionary for reading and updating, they have the same dimension with keys and values. Additionally, our method do not rely on any prior knowledge, such as face parsing and salience detection. 
%$M$ is initialized randomly.

\subsubsection{Self-Supervised Updating}
To learn the patterns of cross domain feature transfer, the memory dictionary $M$ is designed with a self-supervised updating strategy according to the cosine similarity of input feature slots and dictionary items.
The $M$ is initialized randomly.

We employs $F_{p}$ to update the keys and $F_{s}$ to update the values in $M$. 
The keys and values are updated in the same strategy synchronously.
As an illustration to update the keys,  we  firstly compute the cosine similarity $sim_{ij}$ of the $i$th photo feature $f_{i}$ and $j$th key $k_{j}$, in which the similarity is defined as
\begin{equation}\label{4}
sim_{ij}(F_{p},M)=\frac{f_{i}\cdot  k_{j}}{\left \| f_{i} \right \| \left \| k_{j} \right \| }  
\end{equation}
Then, we could find the most relevant key $k_{max}$ for $f_{i}$ which satisfies:
\begin{equation}\label{5}
\phi_{i}  = \mathop{\arg\max}\limits_{j}(sim_{ij})
\end{equation}
For multiple abstract features in $F_{s}$ could refer to the same key, we employ all of them to update the certain key. 
Therefore, we update the memory key $k_{max}$ by
\begin{equation}\label{6}
k_{max}\longleftarrow \alpha\cdot  k_{max} + (1-\alpha )\cdot \frac{\sum_{i=1}^{N}\sum_{j=1}^{K}\mathbbm{1}(k_{j}\in \phi_{i})\cdot f_{i} }{\sum_{i=1}^{N}\sum_{j=1}^{K}\mathbbm{1}(k_{j}\in \phi_{i})} 
\end{equation}
where $\alpha \in \left [ 0,1 \right ] $ is a decay rate.
$N$ is the total number of the photo features.
$K$ is the volume of the dictionary.
The values in $M$ are updated with the same strategy as above.

During each iteration, no additional labels are required. 
Therefore, the proposed memory dictionary is renovated in a self-supervised manner. 
Furthermore, to align the paired features in keys and values, we also propose a novel Memory Refinement loss, of which detailed information is presented in Sec. \ref{MRlossSection}. 

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.5]{MRLOSS2.png}
    \caption{Illustration of the Memory Refinement Loss for feature alignment in the memory module. Two cross domain feature vectors with same spatial information tend to update one pair of key and value in particular. This refinement loss ensures that photo features and sketch features are spatially aligned.}
    \label{fig:MRLoss}
\end{figure}
%这个图示不是很清楚。还是没解释清楚，建议重新整理一下思路，突出体现如何将 key和 value 对齐 spatial


\subsubsection{Attentive Reading}
After updating $M$, we reconstruct sketch feature $\hat{F}_{s}$ by reading the memory items through the query $F_{p}$. Intuitively, it is reasonable to select the most similar memory keys $k_{j}$ and its paired values to reconstruct $F_{p}$. However, it is intractable to back-propagate gradients from decoder to encoders\cite{huang2021memory}. 
On the other hand, as a small part of entire memory dictionary, the single item is lack of style information of sketch images domain. 
%上面这句话是否合理？最好加个引用
To tackle these problems, we proposed an attentive reading strategy for retrieving $\hat{F}_{s}$. 
Firstly, we compute the similarity matrix $S = \left \{ s_{ij}|i=1,\cdots N, j=1,\cdots K  \right \} $ through Eq.\ref{1} with the updated $M$ again. Then, the attention $A = \left \{ a_{ij}|i=1,\cdots N, j=1,\cdots K  \right \}$ is formulated by a softmax operation:
\begin{equation}\label{9}
    a_{ij} = \frac{exp(s_{ij})}{ {\textstyle \sum_{j=1}^{K}exp(s_{ij})} } 
\end{equation}
Afterwards, the retrieved sketch feature $\hat{f}_{i}$ are obtained by
\begin{equation}
    \hat{f}_{i}=\sum_{j}^{K}a_{ij}\cdot v_{j}
\end{equation}
Finally, we aggregate all the retrieved slots to formulate final sketch representation
\begin{equation}
\hat{F}_{s}= \left \{ \hat{f}_{1}, \hat{f}_{2},\hat{f}_{3},\cdots \hat{f}_{N}\right \},\hat{f}_{i} \in \mathbb{R}^{c} 
\end{equation}
Note that during memory reading, $M$ is not updated using back-propagated gradients.

\subsection{Objective Functions}
The overall objective of proposed model includes five loss functions: $\mathcal{L}_{ADV}$, $\mathcal{L}_{rec}$, $\mathcal{L}_{content}$, $\mathcal{L}_{style}$, and $\mathcal{L}_{MR}$. 
%Excluding MR Loss has been discussed in detail, 
In this section, we present these loss functions in detail.
\subsubsection{Adversarial learning} The adversarial loss is leveraged to correctly distinguish the real sketches or generated sketches. As mentioned in Sec. \ref{networkArchitectures}, following \cite{isola2017image}, the adversarial loss is formulated as:
\begin{equation}
\begin{aligned}
    \mathcal{L}_{ADV} &= E_{X,Y}[logD(X,Y)] \\
                    &+ E_{X}[log(1-D(X,G(X))]
\end{aligned}
\end{equation}
where X,Y denote the source photos, target sketches, G,D denote the generator and discriminator.

\subsubsection{Image Reconstruction} As an image-to-image translation task, we expect that the generated sketch could be same as the
ground-truth as possible. 
Therefore, L1 distance is employed to represent the reconstruction loss, defined as 
\begin{equation}
    \mathcal{L}_{rec} = E_{X,Y}[\left \| Y-G(X) \right \|_{1} ]
\end{equation}

\subsubsection{Content and Style Consistency}
In order to ensure that the synthesized sketch and the target sketch have homogeneous style while synethesized sketch and the input photo have similar content, we employ pre-trained VGG-19\cite{simonyan2014very} to extract multi-level representations. 
In terms of fake sketch $G(X)$ and target sketch $Y$, we compute the L2 distance of features from VGG-19 after pool1 and pool2 as Style Loss:
\begin{equation}
\mathcal{L}_{style} = \sum_{i}^{2}\left \|\varphi^{i}(Y) - \varphi^{i}(G(X)) \right \|_{2}^{2}  
\end{equation}
where $\varphi^{i}(cdot)$ represets the output featurrs of VGG-19 net and $i$ denotes the $i$th pool layer of VGG-19 net. 
Additionally, we compute L2 distance of $X$ and $G(x)$ from VGG-19 after pool4 as the Content Loss:
\begin{equation}
\mathcal{L}_{content} =  \left \|\varphi^{4}(Y) - \varphi^{4}(G(X)) \right \|_{2}^{2}  
\end{equation}
The style loss and content loss make training procedure more stable.
%这个stable 你怎么证明呢？建议有曲线，但其实也无所谓。。毕竟6页会议。要是顶会，肯定有人怼你。

==> MOST-NET ICPR2022/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> MemoryDictionary.tex <==
\subsection{Memory Dictionary}
%照应一下A中的命名呗,尽量小模块不用networks，和大的网络冲突
\label{memory}
\subsubsection{Memory Mechanism}
We define the memory mechanism as a dictionary $M$ holding pairs of the key $k_{i}\in \mathbb{R}^{c}$ and value  $v_{i}\in \mathbb{R}^{c}$, which represents the photo feature slots and its corresponding sketch feature slots.
%学术论文最好不用动名词doing开头的句子，主谓宾， 谁干了什么，这种最好
Each entry $(k_{i},v_{i})$ of $M$ represents a feature mapping from photo domain to sketch domain. 
Therefore, a dictionary $M$ containing K items can be described in the following:
\begin{equation}\label{1}
M = \left \{ (k_{i},v_{i})\mid k_{i},v_{i}\in\mathbb{R}^{c},i=1,2,3\cdots ,K \right \}
\end{equation}

Given input photo features $F_{p}$ and sketch features $F_{s}$, we divide them into a number of slots:
\begin{equation}\label{2}
F_{p}= \left \{ f_{1}, f_{2},f_{3},\cdots f_{N}\right \},f_{i}\in \mathbb{R}^{c} 
\end{equation}
\begin{equation}\label{3}
F_{s}= \left \{ s_{1}, s_{2},s_{3},\cdots s_{N}\right \},s_{i}\in \mathbb{R}^{c}
\end{equation}
where $N$ is the number of slots (feature map size), $c$ denotes the dimension of the each slot. Since these slots are intended to interact with Memory Dictionary for reading and updating, they have the same dimension with keys and values. Additionally, our method do not rely on any prior knowledge, such as face parsing and salience detection. 
%$M$ is initialized randomly.

\subsubsection{Self-Supervised Updating}
To learn the patterns of cross domain feature transfer, the memory dictionary $M$ is designed with a self-supervised updating strategy according to the cosine similarity of input feature slots and dictionary items.
The $M$ is initialized randomly.

We employs $F_{p}$ to update the keys and $F_{s}$ to update the values in $M$. 
The keys and values are updated in the same strategy synchronously.
As an illustration to update the keys,  we  firstly compute the cosine similarity $sim_{ij}$ of the $i$th photo feature $f_{i}$ and $j$th key $k_{j}$, in which the similarity is defined as
\begin{equation}\label{4}
sim_{ij}(F_{p},M)=\frac{f_{i}\cdot  k_{j}}{\left \| f_{i} \right \| \left \| k_{j} \right \| }  
\end{equation}
Then, we could find the most relevant key $k_{max}$ for $f_{i}$ which satisfies:
\begin{equation}\label{5}
\phi_{i}  = \mathop{\arg\max}\limits_{j}(sim_{ij})
\end{equation}
For multiple abstract features in $F_{s}$ could refer to the same key, we employ all of them to update the certain key. 
Therefore, we update the memory key $k_{max}$ by
\begin{equation}\label{6}
k_{max}\longleftarrow \alpha\cdot  k_{max} + (1-\alpha )\cdot \frac{\sum_{i=1}^{N}\sum_{j=1}^{K}\mathbbm{1}(k_{j}\in \phi_{i})\cdot f_{i} }{\sum_{i=1}^{N}\sum_{j=1}^{K}\mathbbm{1}(k_{j}\in \phi_{i})} 
\end{equation}
where $\alpha \in \left [ 0,1 \right ] $ is a decay rate.
$N$ is the total number of the photo features.
$K$ is the volume of the dictionary.
The values in $M$ are updated with the same strategy as above.

During each iteration, no additional labels are required. 
Therefore, the proposed memory dictionary is renovated in a self-supervised manner. 
Furthermore, to align the paired features in keys and values, we also propose a novel Memory Refinement loss, of which detailed information is presented in Sec. \ref{MRlossSection}. 

\begin{figure}[t]
    \centering
    \includegraphics[scale=0.5]{MRLOSS2.png}
    \caption{Illustration of the Memory Refinement Loss for feature alignment in the memory module. Two cross domain feature vectors with same spatial information tend to update one pair of key and value in particular. This refinement loss ensures that photo features and sketch features are spatially aligned.}
    \label{fig:MRLoss}
\end{figure}
%这个图示不是很清楚。还是没解释清楚，建议重新整理一下思路，突出体现如何将 key和 value 对齐 spatial


\subsubsection{Attentive Reading}
After updating $M$, we reconstruct sketch feature $\hat{F}_{s}$ by reading the memory items through the query $F_{p}$. Intuitively, it is reasonable to select the most similar memory keys $k_{j}$ and its paired values to reconstruct $F_{p}$. However, it is intractable to back-propagate gradients from decoder to encoders\cite{huang2021memory}. 
On the other hand, as a small part of entire memory dictionary, the single item is lack of style information of sketch images domain. 
%上面这句话是否合理？最好加个引用
To tackle these problems, we proposed an attentive reading strategy for retrieving $\hat{F}_{s}$. 
Firstly, we compute the similarity matrix $S = \left \{ s_{ij}|i=1,\cdots N, j=1,\cdots K  \right \} $ through Eq.\ref{1} with the updated $M$ again. Then, the attention $A = \left \{ a_{ij}|i=1,\cdots N, j=1,\cdots K  \right \}$ is formulated by a softmax operation:
\begin{equation}\label{9}
    a_{ij} = \frac{exp(s_{ij})}{ {\textstyle \sum_{j=1}^{K}exp(s_{ij})} } 
\end{equation}
Afterwards, the retrieved sketch feature $\hat{f}_{i}$ are obtained by
\begin{equation}
    \hat{f}_{i}=\sum_{j}^{K}a_{ij}\cdot v_{j}
\end{equation}
Finally, we aggregate all the retrieved slots to formulate final sketch representation
\begin{equation}
\hat{F}_{s}= \left \{ \hat{f}_{1}, \hat{f}_{2},\hat{f}_{3},\cdots \hat{f}_{N}\right \},\hat{f}_{i} \in \mathbb{R}^{c} 
\end{equation}
Note that during memory reading, $M$ is not updated using back-propagated gradients.

\subsection{Objective Functions}
The overall objective of proposed model includes five loss functions: $\mathcal{L}_{ADV}$, $\mathcal{L}_{rec}$, $\mathcal{L}_{content}$, $\mathcal{L}_{style}$, and $\mathcal{L}_{MR}$. 
%Excluding MR Loss has been discussed in detail, 
In this section, we present these loss functions in detail.
\subsubsection{Adversarial learning} The adversarial loss is leveraged to correctly distinguish the real sketches or generated sketches. As mentioned in Sec. \ref{networkArchitectures}, following \cite{isola2017image}, the adversarial loss is formulated as:
\begin{equation}
\begin{aligned}
    \mathcal{L}_{ADV} &= E_{X,Y}[logD(X,Y)] \\
                    &+ E_{X}[log(1-D(X,G(X))]
\end{aligned}
\end{equation}
where X,Y denote the source photos, target sketches, G,D denote the generator and discriminator.

\subsubsection{Image Reconstruction} As an image-to-image translation task, we expect that the generated sketch could be same as the
ground-truth as possible. 
Therefore, L1 distance is employed to represent the reconstruction loss, defined as 
\begin{equation}
    \mathcal{L}_{rec} = E_{X,Y}[\left \| Y-G(X) \right \|_{1} ]
\end{equation}

\subsubsection{Content and Style Consistency}
In order to ensure that the synthesized sketch and the target sketch have homogeneous style while synethesized sketch and the input photo have similar content, we employ pre-trained VGG-19\cite{simonyan2014very} to extract multi-level representations. 
In terms of fake sketch $G(X)$ and target sketch $Y$, we compute the L2 distance of features from VGG-19 after pool1 and pool2 as Style Loss:
\begin{equation}
\mathcal{L}_{style} = \sum_{i}^{2}\left \|\varphi^{i}(Y) - \varphi^{i}(G(X)) \right \|_{2}^{2}  
\end{equation}
where $\varphi^{i}(cdot)$ represets the output featurrs of VGG-19 net and $i$ denotes the $i$th pool layer of VGG-19 net. 
Additionally, we compute L2 distance of $X$ and $G(x)$ from VGG-19 after pool4 as the Content Loss:
\begin{equation}
\mathcal{L}_{content} =  \left \|\varphi^{4}(Y) - \varphi^{4}(G(X)) \right \|_{2}^{2}  
\end{equation}
The style loss and content loss make training procedure more stable.
%这个stable 你怎么证明呢？建议有曲线，但其实也无所谓。。毕竟6页会议。要是顶会，肯定有人怼你。

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************

